Decoding In-Context Learning: Neuroscience-inspired Analysis of Representations in Large Language Models

Large language models (LLMs) exhibit remarkable performance improvement through in-context learning (ICL) by leveraging task-specific examples in the input. However, the mechanisms behind this improvement remain elusive. In this work, we investigate how LLM embeddings and attention representations change following in-context-learning, and how these changes mediate improvement in behavior. We employ neuroscience-inspired techniques such as representational similarity analysis (RSA) and propose novel methods for parameterized probing and measuring ratio of attention to relevant vs. irrelevant information in Llama-2 70B and Vicuna 13B. We designed two tasks with a priori relationships among their conditions: linear regression and reading comprehension. We formed hypotheses about expected similarities in task representations and measured hypothesis alignment of LLM representations before and after ICL as well as changes in attention. Our analyses revealed a meaningful correlation between improvements in behavior after ICL and changes in both embeddings and attention weights across LLM layers. This empirical framework empowers a nuanced understanding of how latent representations shape LLM behavior, offering valuable tools and insights for future research and practical applications.

==> GraphSection.tex <==
\section{Graph Traversal}
\label{sec:graph_traversal}

The experiments discussed in this section are based on task prompts proposed by ~\cite{cogeval}, where the authors reported failure modes on planning tasks in modern LLMs. Here we used a subset of their tasks, i.e., graph traversal on four graphs, to investigate the effects of ICL on improving planning behavior in LLMs. Moreover, we analyzed latent representations of the first, middle, and last layer of each LLM before and after ICL, and measured the correlation between changes in representations and improvements in planning behavior on graph traversal tasks.

The authors in~\cite{cogeval} investigated whether state-of-the-art LLMs correctly infer the latent structure of different planning problems, known as cognitive maps \cite{Momennejad2020-ey}, and use it for planning. A cognitive map is a representation of latent relational structures that underlie a task in a learning environment, and supports decision-making, reasoning, and deduction in both biological and artificial agents \cite{Tolman1948, Behrens2018-xt, Momennejad2020-ey, Brunec2021-ms}. Such representations also emerge in model-based ~\cite{sutton2018reinforcement} or goal-oriented model-free reinforcement learning (RL)~\cite{lcnfq, plmdp, certified_lcrl_aij, hasanbeig2023symbolic}, to capture a latent construct of the task. 

\newcommand{\scale}{0.13}
\begin{figure}[!t]
\centering
    \subfigure[n7line]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line.png}
        \label{sub_fig:n7line}} 
    \subfigure[n7tree]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree.png}
        \label{sub_fig:n7tree}} 
    \subfigure[n13line]{
        \includegraphics[width=0.2\textwidth]{figs/cogeval/cogeval_n13line.png}
        \label{sub_fig:n13line}}
    \subfigure[n16cluster]{
        \includegraphics[width=0.13\textwidth]{figs/cogeval/cogeval_n16cluster.png}
        \label{sub_fig:n16cluster}}
\caption{\textbf{Graph structure of cognitive maps.} (a) a line graph from \cite{Momennejad2017-wr}. (b) a tree graphs based on \cite{Momennejad2018-zd}. (c) the graph in (a) with double depth from \cite{cogeval} (d) a community graph from \cite{Momennejad2019-tf}.}
\label{fig:cogeval_graphs}
\end{figure}

The prompts are rooted in four MDPs (Figure~\ref{fig:cogeval_graphs}), which are inspired by earlier human reinforcement learning experiments in~\cite{Momennejad2017-wr,Momennejad2018-zd,Momennejad2019-tf,cogeval,allure}. The experiments in this section follow methodological best practices suggested by cognitive scientists \cite{Frank_2023-gx}. Specifically, this section evaluates several graph-traversal tasks, varying graph structure, and domain (sptial rooms with ordered numbers and social ties graph representation), and also using multiple generations (3 generations per condition). These perturbations allow us to robustly measure changes in planning behavior of Llama-2 and Vicuna-1.3 before and after ICL and the corresponding changes in their latent representations. 

We provide examples of task prompts in the supplementary materials (Section~\ref{sec:appendix_cogeval_exp_design}). Improtantly, a correct response to these task prompts requires an understanding of the start and end nodes, comparison of the paths to find the shortest path, and planning a multi-step navigation or traversal of the underlying graph structure of the task. Collectively, we have four graph traversal tasks summarized in the supplementary materials (Table~\ref{tab:conditions_explanation} in Section~\ref{sec:appendix_cogeval_exp_design}). To measure each LLM planning ability more robustly, we constructed five different prompts each with different starting node and goal node. Further to this, we measure the results for each combination of factors and parameters 3 times.

The ICL example that we employed in this experiment is expressed in the ``ordRooms" domain, and explains a step-by-step solution only for a 1-hop policy example:

\begin{framed}
    {\scriptsize You are an AI assistant that helps people find information. You will receive a task and think step by step. Example 1: From room 2 what is the shortest path to room 4? Starting from room 2, please list the room numbers in order, including 2, separated by commas. Here is the sequence of steps from the starting room to the destination room: Go from room 2 to room 4. Answer: 2, 4 $\backslash$n Task:}
\end{framed}

\renewcommand{\scale}{0.2}
\begin{figure}[!t]
\centering
    \subfigure[ordRooms]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_ordRooms_llama2.png}
        \label{sub_fig:ordRooms_llama2_beh}} 
    \subfigure[unordSpatial]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_unordSpatial_llama2.png}
        \label{sub_fig:unordSpatial_llama2_beh}} 
    \subfigure[socialTies]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_socialTies_llama2.png}
        \label{sub_fig:socialTies_llama2_beh}}
    \subfigure[aggregated across domains]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_all_llama2.png}
        \includegraphics[width=0.1\textwidth]{figs/cogeval/graphs_legend.png}
        \label{sub_fig:all_llama2_beh}}
\caption{\textbf{Llama-2 planning behavior in graph traversal task over cognitive graphs and across domains.} The effect of the ICL example on the cognitive maps in Figure~\ref{fig:cogeval_graphs}, when these graphs are expressed in (a) ordRooms, (b) unordSpatial, and (c) socialTies domain. (d) aggregated results}
\label{fig:cogeval_llama2_beh}
\end{figure}

\renewcommand{\scale}{0.22}
\begin{figure}[!t]
\centering
    % \subfigure[transition matrix]{
    %     \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_hypothesisTR.png}
    %     \label{sub_fig:}}  
    \subfigure[first layer w/o ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL0_Llama2_layer0.png}
        \label{sub_fig:llama2_middle_layer_icl_0}}
    \subfigure[first layer w/ ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL1_Llama2_layer0.png}
        \label{sub_fig:llama2_middle_layer_icl_1}}
    \subfigure[middle layer w/o ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL0_Llama2_layer1.png}
        \label{sub_fig:llama2_middle_layer_icl_0}}
    \subfigure[middle layer w/ ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL1_Llama2_layer1.png}
        \label{sub_fig:llama2_middle_layer_icl_1}}
    \subfigure[last layer w/o ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL0_Llama2_layer2.png}
        \label{sub_fig:llama2_last_layer_icl_0}}
    \subfigure[last layer w/ ICL]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_embedding_ICL1_Llama2_layer2.png}
        \label{sub_fig:llama2_last_layer_icl_1}}
    \subfigure[H: successor rep.]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_hypothesisSR.png}
        \label{sub_fig:n7line_hypothesis}}
    \subfigure[emb. vs behavior]{
        \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_emb_delta_w_hyp.png}
        \label{sub_fig:emb_vs_beh_corr}} 
\caption{\textbf{Pairwise embedding similarity analysis of Llama-2 for n7line.} (a)-(f) embedding similarity matrices before and after ICL. ICL has minimal impact on the first layer while the change in the middle layer and the last layer was more significant (g) our hypothesis matrix, i.e., the successor representation for n7line (h) as the correlation between the embeddings similarity matrices (M) and the hypothesis (H) increases, the behavioral success rate improves.}
\label{fig:n7line_rsa}
\end{figure}

where $\backslash$n is the ``new line" special character. The success rates results are presented in Figure~\ref{fig:cogeval_llama2_beh} (and Figure~\ref{fig:cogeval_vicuna_beh} in the supplimentary materials), where we observed significant improvement in the performance of each model, and for each cognitive graph. 

% \renewcommand{\scale}{0.2}
% \begin{figure}[!t]
% \centering
%     \subfigure[ordRooms domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_ordRooms_vicuna.png}
%         \label{sub_fig:ordRooms_vicuna_beh}} 
%     \subfigure[unordSpatial domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_unordSpatial_vicuna.png}
%         \label{sub_fig:unordSpatial_vicuna_beh}} 
%     \subfigure[socialTies domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_socialTies_vicuna.png}
%         \label{sub_fig:socialTies_vicuna_beh}}
%     \subfigure[aggregated across domains]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_all_vicuna.png}
%         \includegraphics[width=0.1\textwidth]{figs/cogeval/graphs_legend.png}
%         \label{sub_fig:all_vicuna_beh}}
% \caption{Vicuna success rate in graph traversal task over cognitive graphs and across domains. The effect of the added ICL example on the cognitive maps in Figure~\ref{fig:cogeval_graphs}, when these graphs are expressed in (a) ordRooms domain, (b) unordSpatial domain, and (c) socialTies domain. The aggregated results are shown in (d).}
% \label{fig:cogeval_vicuna_beh}
% \end{figure}

% \renewcommand{\scale}{0.2}
% \begin{figure}[!t]
% \centering
%     \subfigure[ordRooms domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_condition_ordRooms_llama2.png}
%         \label{sub_fig:ordRooms_llama2_beh_cond}} 
%     \subfigure[unordSpatial domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_condition_unordSpatial_llama2.png}
%         \label{sub_fig:unordSpatial_llama2_beh_cond}} 
%     \subfigure[socialTies domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_condition_socialTies_llama2.png}
%         \label{sub_fig:socialTies_llama2_beh_cond}}
%     \subfigure[aggregated across domains]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_condition_all_llama2.png}
%         \includegraphics[width=0.1\textwidth]{figs/cogeval/tasks_legend.png}
%         \label{sub_fig:all_llama2_beh_cond}}
% \caption{Llama-2 success rate in graph traversal task over tasks and across domains. The effect of the added ICL example on the cognitive maps in Figure~\ref{fig:cogeval_graphs}, when these graphs are expressed in (a) ordRooms domain, (b) unordSpatial domain, and (c) socialTies domain. The aggregated results are shown in (d).}
% \label{fig:cogeval_llama2_beh_cond}
% \end{figure}

% \renewcommand{\scale}{0.2}
% \begin{figure}[!t]
% \centering
%     \subfigure[ordRooms domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_ordRooms_vicuna.png}
%         \label{sub_fig:ordRooms_vicuna_beh_cond}} 
%     \subfigure[unordSpatial domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_unordSpatial_vicuna.png}
%         \label{sub_fig:unordSpatial_vicuna_beh_cond}} 
%     \subfigure[socialTies domain]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_socialTies_vicuna.png}
%         \label{sub_fig:socialTies_vicuna_beh_cond}}
%     \subfigure[aggregated across domains]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_behavior_all_vicuna.png}
%         \includegraphics[width=0.1\textwidth]{figs/cogeval/tasks_legend.png}
%         \label{sub_fig:all_vicuna_beh_cond}}
% \caption{Vicuna success rate in graph traversal task over tasks and across domains. The effect of the added ICL example on the cognitive maps in Figure~\ref{fig:cogeval_graphs}, when these graphs are expressed in (a) ordRooms domain, (b) unordSpatial domain, and (c) socialTies domain. The aggregated results are shown in (d).}
% \label{fig:cogeval_vicuna_beh_cond}
% \end{figure}
  
% \subsection{RSA}
\textbf{RSA:} These findings encouraged us to look deeper into the representational changes inside each model and to examine whether there is a meaningful correlation between such changes and the improvements we observed in the performance. Specifically, we opened the models at different layers and looked into the embeddings representations to study the changes in the neural embeddings before and after ICL, e.g., Figure~\ref{fig:n7line_rsa}(a)-(f) for n7line. Our hypothesis is that the model's behavioral performance improves after ICL due to the model's finer perception of the graph structures. To assess this hypothesis, we adopted the graphs' successor representation matrices (Figure~\ref{sub_fig:n7line_hypothesis}), which capture the actual similarities between the nodes of each graph, and compared the successor representation matrices with the pairwise cosine similarity matrices that capture the similarity of the graph nodes embeddings. We found out that there is a positive correlation between the similarity of the embeddings and the successor representation, and the success rate of the model.  

% \renewcommand{\scale}{0.23}
% \begin{figure}[!t]
% \centering
%     \subfigure[transition matrix]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_hypothesisTR.png}
%         \label{sub_fig:}} 
%     \subfigure[successor representation]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line_hypothesisSR.png}
%         \label{sub_fig:}} 
%     \subfigure[first layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL0_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[first layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL1_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL0_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL1_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[last layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL0_Llama2_layer2.png}
%         \label{sub_fig:}}
%     \subfigure[last layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_social_n7line_embedding_ICL1_Llama2_layer2.png}
%         \label{sub_fig:}}
% \caption{Llama-2 all layers for n7line}
% \label{fig:}
% \end{figure}

% \renewcommand{\scale}{0.23}
% \begin{figure}[!t]
% \centering
%     \subfigure[transition matrix]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_hypothesisTR.png}
%         \label{sub_fig:}} 
%     \subfigure[successor representation]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_hypothesisSR.png}
%         \label{sub_fig:}} 
%     \subfigure[first layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL0_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[first layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL1_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL0_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL1_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[last layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL0_Llama2_layer2.png}
%         \label{sub_fig:}}
%     \subfigure[last layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree_embedding_ICL1_Llama2_layer2.png}
%         \label{sub_fig:}}
% \caption{Llama-2 all layers for n7tree}
% \label{fig:}
% \end{figure}

% \renewcommand{\scale}{0.23}
% \begin{figure}[!t]
% \centering
%     \subfigure[transition matrix]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_hypothesisTR.png}
%         \label{sub_fig:}} 
%     \subfigure[successor representation]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_hypothesisSR.png}
%         \label{sub_fig:}} 
%     \subfigure[first layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL0_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[first layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL1_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL0_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL1_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[last layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL0_Llama2_layer2.png}
%         \label{sub_fig:}}
%     \subfigure[last layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n13line_embedding_ICL1_Llama2_layer2.png}
%         \label{sub_fig:}}
% \caption{Llama-2 all layers for n13line}
% \label{fig:}
% \end{figure}

% \renewcommand{\scale}{0.23}
% \begin{figure}[!t]
% \centering
%     \subfigure[transition matrix]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_hypothesisTR.png}
%         \label{sub_fig:}} 
%     \subfigure[successor representation]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_hypothesisSR.png}
%         \label{sub_fig:}} 
%     \subfigure[first layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL0_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[first layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL1_Llama2_layer0.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL0_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[middle layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL1_Llama2_layer1.png}
%         \label{sub_fig:}}
%     \subfigure[last layer before ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL0_Llama2_layer2.png}
%         \label{sub_fig:}}
%     \subfigure[last layer after ICL]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster_embedding_ICL1_Llama2_layer2.png}
%         \label{sub_fig:}}
% \caption{Llama-2 all layers for n16cluster}
% \label{fig:}
% \end{figure}

% \renewcommand{\scale}{0.18}
% \begin{figure}[!t]
% \centering
%     \subfigure[]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7line.png}
%         \label{sub_fig:}} 
%     \subfigure[]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n7tree.png}
%         \label{sub_fig:}} 
%     \subfigure[]{
%         \includegraphics[width=0.3\textwidth]{figs/cogeval/cogeval_n13line.png}
%         \label{sub_fig:}}
%     \subfigure[]{
%         \includegraphics[width=\scale\textwidth]{figs/cogeval/cogeval_n16cluster.png}
%         \label{sub_fig:}}
% \caption{}
% \label{fig:}
% \end{figure}

